The NANOGrav 12.5-year Data Set: Wideband Timing of 47 Millisecond Pulsars

We present a new analysis of the profile data from the 47 millisecond pulsars comprising the 12.5-year data set of the North American Nanohertz Observatory for Gravitational Waves (NANOGrav), which is presented in a parallel paper (Alam et al. 2021a; NG12.5). Our reprocessing is performed using "wideband" timing methods, which use frequency-dependent template profiles, simultaneous time-of-arrival (TOA) and dispersion measure (DM) measurements from broadband observations, and novel analysis techniques. In particular, the wideband DM measurements are used to constrain the DM portion of the timing model. We compare the ensemble timing results to NG12.5 by examining the timing residuals, timing models, and noise model components. There is a remarkable level of agreement across all metrics considered. Our best-timed pulsars produce encouragingly similar results to those from NG12.5. In certain cases, such as high-DM pulsars with profile broadening, or sources that are weak and scintillating, wideband timing techniques prove to be beneficial, leading to more precise timing model parameters by 10-15%. The high-precision, multi-band measurements of several pulsars indicate frequency-dependent DMs. Compared to the narrowband analysis in NG12.5, the TOA volume is reduced by a factor of 33, which may ultimately facilitate computational speed-ups for complex pulsar timing array analyses. This first wideband pulsar timing data set is a stepping stone, and its consistent results with NG12.5 assure us that such data sets are appropriate for gravitational wave analyses.

==> tables/tab_flux.tex <==
\begin{deluxetable}{@{\extracolsep{35pt}}cll}[ht!]
  \tabletypesize{\footnotesize}
  \tablewidth{\columnwidth}
  \tablecaption{Mean Flux Densities \& Spectral Indices\label{tab:flux}}
  \tablehead{\colhead{Source} & \colhead{$S_{1400}$} & \colhead{Index} \\[-8pt] \colhead{} & \colhead{\hspace*{0pt}\hfill [mJy]} & \colhead{}}
    \startdata
      J0023$+$0923  &  \phantom{1}1.6(1)  &  $-1.2$(2)\phn \\
      J0030$+$0451  &  \phantom{1}1.43(9)  &  $-2.2$(2)\phn \\
      J0340$+$4130  &  \phantom{1}0.62(1)  &  $-1.72$(3)\phn \\
      J0613$-$0200  &  \phantom{1}2.84(5)  &  $-1.83$(3)\phn \\
      J0636$+$5128  &  \phantom{1}1.50(4)  &  $-1.48$(7)\phn \\
      J0645$+$5158  &  \phantom{1}1.2(2)  &  $-4.8$(4)\phn \\
      J0740$+$6620  &  \phantom{1}2.36(8)  &  $-2.27$(8)\phn \\
      J0931$-$1902  &  \phantom{1}1.58(7)  &  $-1.3$(1)\phn \\
      J1012$+$5307  &  \phantom{1}8.6(5)  &  $-2.6$(2)\phn \\
      J1024$-$0719  &  \phantom{1}3.4(1)  &  $-3.2$(2)\phn \\
      J1125$+$7819  &  \phantom{1}2.9(2)  &  $-2.0$(1)\phn \\
      J1453$+$1902  &  \phantom{1}0.52(9)  &  $-1.7$(4)\phn \\
      J1455$-$3330  &  \phantom{1}2.1(1)  &  $-2.3$(2)\phn \\
      J1600$-$3053  &  \phantom{1}2.66(2)  &  $-0.51$(1)\phn \\
      J1614$-$2230  &  \phantom{1}1.71(4)  &  $-1.26$(4)\phn \\
      J1640$+$2224  &  \phantom{1}2.5(1)  &  $-1.69$(7)\phn \\
      J1643$-$1224  &  \phantom{1}5.0(1)  &  $-1.72$(4)\phn \\
      J1713$+$0747  &  16.5(6)  &  $-0.8$(1)\phn \\
      J1738$+$0333  &  \phantom{1}1.7(1)  &  $-0.8$(2)\phn \\
      J1741$+$1351  &  \phantom{1}1.13(5)  &  $-1.42$(5)\phn \\
      J1744$-$1134  &  \phantom{1}8.2(3)  &  $-2.05$(7)\phn \\
      J1747$-$4036  &  \phantom{1}1.81(2)  &  $-2.54$(2)\phn \\
      J1832$-$0836  &  \phantom{1}1.35(2)  &  $-1.73$(5)\phn \\
      J1853$+$1303  &  \phantom{1}1.07(4)  &  $-1.42$(5)\phn \\
      B1855$+$09\phantom{....}  &  \phantom{1}9.6(5)  &  $-0.60$(4)\phn \\
      J1903$+$0327  &  \phantom{1}0.83(5)  &  $-1.6$(3)\phn \\
      J1909$-$3744  &  \phantom{1}6.7(2)  &  $-0.81$(6)\phn \\
      J1910$+$1256  &  \phantom{1}0.76(1)  &  $-0.95$(8)\phn \\
      J1911$+$1347  &  \phantom{1}1.52(4)  &  $-0.65$(2)\phn \\
      J1918$-$0642  &  \phantom{1}3.6(1)  &  $-1.49$(7)\phn \\
      J1923$+$2515  &  \phantom{1}0.92(3)  &  $-1.17$(4)\phn \\
      B1937$+$21\phantom{....}  &  16.7(2)  &  $-2.12$(5)\phn \\
      J1944$+$0907  &  \phantom{1}5.1(2)  &  $-1.32$(3)\phn \\
      J1946$+$3417  &  \phantom{1}0.93(1)  &  $-1.20$(3)\phn \\
      B1953$+$29\phantom{....}  &  \phantom{1}1.04(2)  &  $-2.00$(6)\phn \\
      J2010$-$1323  &  \phantom{1}1.27(3)  &  $-1.01$(6)\phn \\
      J2017$+$0603  &  \phantom{1}0.81(6)  &  $-0.3$(1)\phn \\
      J2033$+$1734  &  \phantom{1}0.43(1)  &  $-1.80$(2)\phn \\
      J2043$+$1711  &  \phantom{1}0.84(3)  &  $-1.27$(5)\phn \\
      J2145$-$0750  &  12.1(4)  &  $-3.0$(2)\phn \\
      J2214$+$3000  &  \phantom{1}1.7(2)  &  $-2.4$(3)\phn \\
      J2229$+$2643  &  \phantom{1}1.69(8)  &  $-1.55$(9)\phn \\
      J2234$+$0611  &  \phantom{1}1.6(3)  &  $-0.6$(5)\phn \\
      J2234$+$0944  &  \phantom{1}6.1(7)  &  $-2.5$(4)\phn \\
      J2302$+$4442  &  \phantom{1}2.62(7)  &  $-0.89$(5)\phn \\
      J2317$+$1439  &  \phantom{1}2.2(2)  &  $-1.29$(9)\phn \\
      J2322$+$2057  &  \phantom{1}1.52(7)  &  $-1.2$(1)\phn \\
    \enddata
  \tablecomments{
  The columns list mean flux densities estimated at 1400~MHz and the associated spectral index for power-law functions fit across all observed bands.
  Uncertainties (in parentheses, for the last digit) include the variance in residual structure after fitting power-law functions in each band.
  See \twelveyr\ for a more detailed analysis.
  }
\end{deluxetable}


==> text/fig_prof_evol.tex <==
\begin{figure}[htb!]
%\begin{center}
\includegraphics[width=\columnwidth]{figs/prof_evol.pdf}
\caption{\label{fig:prof_evol}
Schematic of modeling profile evolution; see text for a mathematical description.
The smoothly varying green curve spans the variation drawn out by the evolving red profile (seen here in projection) from some low to some high frequency.
The profile evolution curve is expressed in the basis of the orange profiles, found via PCA.
The frequency-parameterized coordinates of the curve are used to linearly combine the basis eigenprofiles, forming any of the purple difference profiles, which construct a template profile when added to the gray mean profile vector.
}
%\end{center}
\end{figure}


==> text/figset_summary.tex <==
\figsetstart

\figsetnum{9}
\figsettitle{Timing Residuals \& DM Variations}

\figsetgrpstart
\figsetgrpnum{9.1}
\figsetgrptitle{J0023+0923}
\figsetplot{figs/J0023+0923_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J0023$+$0923. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.2}
\figsetgrptitle{J0030+0451}
\figsetplot{figs/J0030+0451_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J0030$+$0451. Colored points indicate the receiver for the observation: 430~MHz (Orange), 1.4~GHz (Light blue), and 2.1~GHz (Purple).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.3}
\figsetgrptitle{J0340+4130}
\figsetplot{figs/J0340+4130_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J0340$+$4130. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.4}
\figsetgrptitle{J0613-0200}
\figsetplot{figs/J0613-0200_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J0613$-$0200. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.5}
\figsetgrptitle{J0636+5128}
\figsetplot{figs/J0636+5128_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J0636$+$5128. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.6}
\figsetgrptitle{J0645+5158}
\figsetplot{figs/J0645+5158_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J0645$+$5158. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.7}
\figsetgrptitle{J0740+6620}
\figsetplot{figs/J0740+6620_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J0740$+$6620. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.8}
\figsetgrptitle{J0931-1902}
\figsetplot{figs/J0931-1902_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J0931$-$1902. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.9}
\figsetgrptitle{J1012+5307}
\figsetplot{figs/J1012+5307_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1012$+$5307. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.10}
\figsetgrptitle{J1024-0719}
\figsetplot{figs/J1024-0719_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1024$-$0719. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.11}
\figsetgrptitle{J1125+7819}
\figsetplot{figs/J1125+7819_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1125$+$7819. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.12}
\figsetgrptitle{J1453+1902}
\figsetplot{figs/J1453+1902_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1453$+$1902. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.13}
\figsetgrptitle{J1455-3330}
\figsetplot{figs/J1455-3330_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1455$-$3330. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.14}
\figsetgrptitle{J1600-3053}
\figsetplot{figs/J1600-3053_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1600$-$3053. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.15}
\figsetgrptitle{J1614-2230}
\figsetplot{figs/J1614-2230_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1614$-$2230. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.16}
\figsetgrptitle{J1640+2224}
\figsetplot{figs/J1640+2224_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1640$+$2224. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.17}
\figsetgrptitle{J1643-1224}
\figsetplot{figs/J1643-1224_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1643$-$1224. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.18}
\figsetgrptitle{J1713+0747}
\figsetplot{figs/J1713+0747_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1713$+$0747. Colored points indicate the receiver for the observation: 820~MHz (Green), 1.4~GHz (Dark blue), 1.4~GHz (Light blue), and 2.1~GHz (Purple).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.19}
\figsetgrptitle{J1738+0333}
\figsetplot{figs/J1738+0333_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1738$+$0333. Colored points indicate the receiver for the observation: 1.4~GHz (Light blue) and 2.1~GHz (Purple).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.20}
\figsetgrptitle{J1741+1351}
\figsetplot{figs/J1741+1351_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1741$+$1351. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.21}
\figsetgrptitle{J1744-1134}
\figsetplot{figs/J1744-1134_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1744$-$1134. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.22}
\figsetgrptitle{J1747-4036}
\figsetplot{figs/J1747-4036_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1747$-$4036. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.23}
\figsetgrptitle{J1832-0836}
\figsetplot{figs/J1832-0836_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1832$-$0836. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.24}
\figsetgrptitle{J1853+1303}
\figsetplot{figs/J1853+1303_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1853$+$1303. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.25}
\figsetgrptitle{B1855+09}
\figsetplot{figs/B1855+09_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for B1855$+$09. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.26}
\figsetgrptitle{J1903+0327}
\figsetplot{figs/J1903+0327_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1903$+$0327. Colored points indicate the receiver for the observation: 1.4~GHz (Light blue) and 2.1~GHz (Purple).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.27}
\figsetgrptitle{J1909-3744}
\figsetplot{figs/J1909-3744_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1909$-$3744. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.28}
\figsetgrptitle{J1910+1256}
\figsetplot{figs/J1910+1256_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1910$+$1256. Colored points indicate the receiver for the observation: 1.4~GHz (Light blue) and 2.1~GHz (Purple).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.29}
\figsetgrptitle{J1911+1347}
\figsetplot{figs/J1911+1347_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1911$+$1347. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.30}
\figsetgrptitle{J1918-0642}
\figsetplot{figs/J1918-0642_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1918$-$0642. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.31}
\figsetgrptitle{J1923+2515}
\figsetplot{figs/J1923+2515_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1923$+$2515. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.32}
\figsetgrptitle{B1937+21}
\figsetplot{figs/B1937+21_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for B1937$+$21. Colored points indicate the receiver for the observation: 820~MHz (Green), 1.4~GHz (Dark blue), 1.4~GHz (Light blue), and 2.1~GHz (Purple).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.33}
\figsetgrptitle{J1944+0907}
\figsetplot{figs/J1944+0907_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1944$+$0907. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.34}
\figsetgrptitle{J1946+3417}
\figsetplot{figs/J1946+3417_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J1946$+$3417. Colored points indicate the receiver for the observation: 1.4~GHz (Light blue) and 2.1~GHz (Purple).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.35}
\figsetgrptitle{B1953+29}
\figsetplot{figs/B1953+29_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for B1953$+$29. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.36}
\figsetgrptitle{J2010-1323}
\figsetplot{figs/J2010-1323_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2010$-$1323. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.37}
\figsetgrptitle{J2017+0603}
\figsetplot{figs/J2017+0603_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2017$+$0603. Colored points indicate the receiver for the observation: 430~MHz (Orange), 1.4~GHz (Light blue), and 2.1~GHz (Purple).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.38}
\figsetgrptitle{J2033+1734}
\figsetplot{figs/J2033+1734_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2033$+$1734. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.39}
\figsetgrptitle{J2043+1711}
\figsetplot{figs/J2043+1711_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2043$+$1711. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.40}
\figsetgrptitle{J2145-0750}
\figsetplot{figs/J2145-0750_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2145$-$0750. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.41}
\figsetgrptitle{J2214+3000}
\figsetplot{figs/J2214+3000_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2214$+$3000. Colored points indicate the receiver for the observation: 1.4~GHz (Light blue) and 2.1~GHz (Purple).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.42}
\figsetgrptitle{J2229+2643}
\figsetplot{figs/J2229+2643_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2229$+$2643. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.43}
\figsetgrptitle{J2234+0611}
\figsetplot{figs/J2234+0611_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2234$+$0611. Colored points indicate the receiver for the observation: 430~MHz (Orange) and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.44}
\figsetgrptitle{J2234+0944}
\figsetplot{figs/J2234+0944_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2234$+$0944. Colored points indicate the receiver for the observation: 1.4~GHz (Light blue) and 2.1~GHz (Purple).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.45}
\figsetgrptitle{J2302+4442}
\figsetplot{figs/J2302+4442_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2302$+$4442. Colored points indicate the receiver for the observation: 820~MHz (Green) and 1.4~GHz (Dark blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.46}
\figsetgrptitle{J2317+1439}
\figsetplot{figs/J2317+1439_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2317$+$1439. Colored points indicate the receiver for the observation: 327~MHz (Red), 430~MHz (Orange), and 1.4~GHz (Light blue).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{9.47}
\figsetgrptitle{J2322+2057}
\figsetplot{figs/J2322+2057_summary.pdf}
\figsetgrpnote{Summary of timing residuals and DM variations for J2322$+$2057. Colored points indicate the receiver for the observation: 430~MHz (Orange), 1.4~GHz (Light blue), and 2.1~GHz (Purple).  Black circles and grey squares in the bottom panel are DMX values; the latter are from \twelveyr.}
\figsetgrpend

\figsetend

